TIGGER: Scalable Generative Modelling for Temporal Interaction Graphs

There has been a recent surge in learning generative models for graphs. While impressive progress has been made on static graphs, work on generative modeling of temporal graphs is at a nascent stage with significant scope for improvement. First, existing generative models do not scale with either the time horizon or the number of nodes. Second, existing techniques are transductive in nature and thus do not facilitate knowledge transfer. Finally, due to relying on one-to-one node mapping from source to the generated graph, existing models leak node identity information and do not allow up-scaling/down-scaling the source graph size. In this paper, we bridge these gaps with a novel generative model called TIGGER. TIGGER derives its power through a combination of temporal point processes with auto-regressive modeling enabling both transductive and inductive variants. Through extensive experiments on real datasets, we establish TIGGER generates graphs of superior fidelity, while also being up to 3 orders of magnitude faster than the state-of-the-art.

==> 1_related_work.tex <==
\todo{remove}
\section{Related Work}
\label{sec:related_work}

\textbf{Static Graphs}

In the recent years, various deep learning based techniques have been proposed for static graph generative modelling. GraphRNN\cite{you2018graphrnn} modelled distribution of static graphs (50-200 nodes) using a node-level and edge-level RNN. GraphGen\cite{goyal2020graphgen} utilizes minimum DFS code \cite{1184038} to represent each graph and is scalable to larger and labelled graphs ($\approx$ 500 nodes). GRAN\cite{liao2020efficient} builds upon the GraphRNN architecture where RNNs are replaced by attention networks removing the long term nodes dependencies. This improves the quality of sampled graphs. Moreover, instead of generating one node at a time, they generate a block of nodes and associated edges at each step. This helps in reducing the sampling time and enables the training over large scale graphs ($\approx$ 5k nodes). NetGAN\cite{bojchevski2018netgan} utilizes a GAN based architecture where the generator learns to generate synthetic random walks while the task of the discriminator is to learn to discriminate synthetic random walks from real random walks. We observe that NetGAN requires a single graph during training while other algorithms require a collection of graphs. Significant progress has been made through these approaches, however all of them are designed only for generating static graphs only.


\textbf{Temporal Graph generation}

Unlike static networks where there are standard graph models like Erdős Rényi graph model \cite{erd1959a} and small world model \cite{watts1998a}, such de-facto models are not present for temporal networks which combine the topology with time. Few works have  attempted to formulate the generation process of network to understand the spreading of diseases via contact using temporal networks. \cite{10.1371/journal.pcbi.1003142} has proposed a approach where they start by generating a static network and for each link in the network, they generate an active time-span and start time. Also, sample sequence of contact times for the network from inter-event time distribution. Finally, they overlay this sequence with active time span of each link to generate a interaction network.  \cite{perra2012a} introduces activity driven temporal network generative approach. At each time-stamp, they start with N disconnected nodes. With probability $p_i$ defined as activity potential, node i becomes active and connect with randomly chosen m nodes. At the next time-stamp same process is repeated. \cite{Vestergaard_2014} proposes a memory based method for both node and link activation. It stores a time since last interaction $\tau_{i}$ for node i and $\tau_{ij}$ for link between node i and j. Initially in a N size network, all nodes are inactive. A node can become active with probability $bf_{node}(\tau_{i})$ and initiate a link with inactive node j with probability  $g_{node}(\tau_{j})g_{link}(\tau_{ij})$. A link can deactive with probability $zf_{link}(\tau_{ij})$. Both $b$ and $z$ are control parameters. $f$ and $g$ are memory kernels of power law distribution. \cite{TagGen} proposed a neural generative model for temporal interaction network by transforming it into a static network by merging node identity with time of interactions to create new time-aware nodes. They further learn a discriminator to differentiate between actual random walks and sampled random walks. Furthermore, they sample a new static network from sampled walks which are classified by the discriminator as real walks. Finally, they convert the sampled static network to temporal interaction network by detaching node identity from time.  Very recent approach DYMOND \cite{10.1145/3442381.3450102} proposes a graphlet based dynamic graph generative approach. They consider graphlets of maximum size 3. At each time step, they first sample active nodes and then sample graphlets consisting of those nodes by estimating arrival rate for each unique graphlet.This approach has $O(N^3)$ complexity due to graphlets extraction making it less suitable for higher size network.


% $\bullet$ \textbf{Inductive node generation}:
% Although \tggan proposed an architecture to generate temporal graphs, however, the approach doesn't perform node generation and assumes the node set is fixed. 


% $\bullet$ \textbf{Large number of unique timestamps}:
% It is not uncommon to find temporal graphs having large number of unique timestamps\todo{add citations}.
% For instance, the Reddit network there are over 60K unique timestamps. \todo{more examples}.
% However, \tggan is limited to temporal graphs of approximately a hundred unique timestamps. Further, it fails to scale to real datasets such as \todo{datasetname} \todo{cite exp section}. \todo{Reason}


% $\bullet$ \textbf{Incorporating node features}:
% Presence of features in nodes are quite common in today's real world graphs \todo{cite datasets} which are used by various graph learning based models to improve performance in downstream tasks. However, existing work on temporal graph generative modelling \tggan doesn't utilize node features and hence ignore information present which could be useful.


